Simultaneous Coverage and Efficiency Guarantee in Online Conformal Prediction

Adaptive conformal inference (ACI) of Gibbs and Cand{\`e}s and its variants are the standard approach to online conformal prediction under distribution shift, but they suffer from three fundamental limitations. First, their guarantees control only the \emph{signed} long-run coverage error: persistent miscoverage in one direction can be masked by compensating errors later, so a method can satisfy the theoretical guarantee while being badly wrong for extended periods. Second, existing guarantees say nothing about prediction-set size, so validity can be achieved trivially at the cost of unduly wide prediction sets. Third, the efficiency guarantees that do exist compare against a \emph{fixed} predictor chosen in hindsight, a benchmark that becomes increasingly less meaningful once the data-generating distribution shifts, since the very notion of an optimal threshold then changes over time. We consider a unified online learning framework that simultaneously controls absolute, non-cancelling coverage violation and prediction-set efficiency against a dynamically evolving benchmark for three important models. In the fully adversarial setting, exploiting the fact that the standard ACI update is exactly projected online gradient descent on the pinball loss, we derive simultaneous coverage and efficiency guarantees for arbitrary monotone Lipschitz efficiency objectives, with no distributional or {\it convexity} assumptions. In the stochastic setting with full-score feedback, we propose a sliding-window quantile tracker and establish a matching minimax lower bound showing our algorithm is rate-optimal. In the covariate-dependent stochastic setting, we develop a partitioned ACI algorithm that tracks a function-valued oracle threshold, and derive simultaneous coverage and efficiency guarantees.

==> technical_part.tex <==
\paragraph{Notation and conventions.}
Throughout: $\alpha\in(0,1)$ is the target miscoverage level;
$A=[0,Q_{\max}]$ is the threshold action space;
$\X=[0,1]^d$ is the covariate space; $T$ is the time horizon.
We use the \textbf{single, fixed convention}
\[
z_t := \mathbf{1}(Y_t\in C_t) = \mathbf{1}(s(X_t,Y_t)\le q_t(X_t)),
\]
so $z_t=1$ means ``covered'' and $\E[z_t|q_t,X_t]=F_t(q_t(X_t)|X_t)$.
In Section~\ref{sec:adversarial} the score $r_t$ is revealed directly;
in Sections~\ref{sec:scalar}--\ref{sec:conditional} the learner sees
only $z_t$.

\paragraph{General problem formulation.}
At each round $t=1,\dots,T$, the learner observes a covariate $X_t\in\X$
(when the model includes covariates), selects a threshold $q_t$, and
forms the prediction set
\[
C_t(X_t)=\{y\in\Y:s(X_t,y)\le q_t\},
\]
incurring an efficiency cost $f_t(q_t):=\mu(C_t(X_t))$, where $\mu(\cdot)$
is an intrinsic measure of prediction-set size (interval length, volume,
or cardinality). After $Y_t$ is revealed, the realized conformity score
$r_t:=s(X_t,Y_t)$ becomes available in the full-feedback models of
Sections~\ref{sec:adversarial}--\ref{sec:scalar}; coverage is achieved
whenever $q_t\ge r_t$, with feasibility violation $(r_t-q_t)_+$.

We measure the learner against any \emph{feasible} dynamic comparator
sequence $u=(u_1,\dots,u_T)$ satisfying $u_t\ge r_t$ for every $t$, and
in particular against the optimal feasible sequence
\[
u^*\in\arg\min_{\{u_t\ge r_t\}}\sum_{t=1}^Tf_t(u_t).
\]
Because each $f_t$ is nondecreasing, the constrained minimizer is
attained pointwise at $u_t^*=r_t$, the smallest threshold achieving
coverage at round $t$. Performance is reported through the
\textbf{dynamic regret}
\[
R(T)=\sum_{t=1}^Tf_t(q_t)-\sum_{t=1}^Tf_t(u_t^*),
\]
and the \textbf{cumulative feasibility violation}
\[
Q(T)=\sum_{t=1}^T(r_t-q_t)_+,
\]
with the goal of achieving $R(T)=o(T)$ and $Q(T)=o(T)$ simultaneously.
This optimization problem is identical across Models~\ref{sec:adversarial}%
--\ref{sec:conditional} below; only the assumptions placed on the
conformity-score process $\{r_t\}$ (or, in
Model~\ref{sec:conditional}, on the joint process $\{(X_t,r_t)\}$)
change. When the learner receives only the coverage bit
$z_t=\mathbf{1}(r_t\le q_t)$ rather than $r_t$ itself
(Models~\ref{sec:scalar}--\ref{sec:conditional}), $r_t$ is no longer
observed and $Q(T)$ is restated directly in terms of the underlying
score distributions; we keep the name $Q(T)$ for this distributional
analogue in Model~\ref{sec:scalar} and write $V_c(T)$ for its
covariate-conditional counterpart in Model~\ref{sec:conditional}, as
defined in each section below.

%==================================================================
\section{Model I: Adversarial Scores with Full Feedback}
\label{sec:adversarial}
%==================================================================

\paragraph{Why start here.}
This is the most permissive model: no distributional assumptions on how
scores are generated, and the learner sees the realized score $r_t$
after each round. It already covers a central question---what is the
structural relationship between ACI and online learning?---and gives the
cleanest result: ACI is literally OGD on a classical loss, with
simultaneous efficiency and coverage guarantees requiring no convexity.
Sections~\ref{sec:scalar} and~\ref{sec:conditional} then impose
distributional structure to obtain sharper rates.

\subsection{Setup}

At each round $t=1,\dots,T$ (a covariate $X_t$ may or may not be
present; here the threshold does not condition on it, so we suppress
it from the notation and work directly with the induced score $r_t$):
\begin{enumerate}[label=(\arabic*)]
\item Learner selects threshold $q_t\in A=[0,Q_{\max}]$.
\item Nature reveals conformity score $r_t\in A$, chosen
      adversarially (no distributional assumption).
\item Learner observes $z_t=\mathbf{1}(r_t\le q_t)$ and incurs
      efficiency cost $f_t(q_t)=\mu(C_t(X_t))$ and coverage shortfall
      $(r_t-q_t)_+$.
\end{enumerate}

\begin{definition}[Performance metrics]
\label{def:adv-metrics}
\[
R(T)=\sum_{t=1}^T\!\bigl(f_t(q_t)-f_t(r_t)\bigr),\quad
Q(T)=\sum_{t=1}^T(r_t-q_t)_+.
\]
These instantiate the general definitions of $R(T)$ and $Q(T)$ from
the problem formulation above: since $f_t$ is nondecreasing, the
feasible comparator minimizing $\sum_tf_t(u_t)$ subject to $u_t\ge r_t$
is attained pointwise at $u_t^*=r_t$, the smallest threshold achieving
coverage at round $t$. Its total variation is
$P_T=\sum_{t=2}^T|r_t-r_{t-1}|$.
\end{definition}

\begin{remark}[Efficiency cost need not be convex]
\label{rem:nonconvex}
The set-size function $\mu(q,x):=\lambda(\{y:s(x,y)\le q\})$ is always
nondecreasing in $q$ (larger threshold $\Rightarrow$ larger set) but is
generically \emph{non-convex}: its derivative $\partial_q\mu$ equals
the marginal score density, which decreases on the left of the mode for
any unimodal distribution (Gaussian, Laplace, etc.). Demanding convexity
would rule out the most natural efficiency costs. Our result requires
only monotonicity and Lipschitz continuity.
\end{remark}

\subsection{The Pinball Loss and Its Connection to ACI}

\begin{definition}[Pinball (quantile) loss]
\[
\psi_t(q):=(1-\alpha)(r_t-q)_++\alpha(q-r_t)_+.
\]
This is the standard quantile regression loss targeting the
$(1-\alpha)$-quantile of $r_t$.
\end{definition}

\begin{theorem}[ACI is OGD on pinball losses]
\label{thm:adversarial}
Let $f_t:A\to\R$ be any monotone nondecreasing $L$-Lipschitz function
(not necessarily convex). Consider the ACI update with step size
$\eta>0$:
\[
q_{t+1}=\Pi_A\!\bigl[q_t+\eta\bigl((1-z_t)-\alpha\bigr)\bigr].
\]
\begin{enumerate}[label=(\roman*)]
\item \textbf{(ACI = OGD on pinball).}
      This update is exactly projected online gradient descent with
      step size $\eta$ applied to the pinball losses $\{\psi_t\}$:
      $q_{t+1}=\Pi_A[q_t-\eta\,\tilde{g}_t]$ for
      $\tilde{g}_t\in\partial\psi_t(q_t)$.
\item \textbf{(Dynamic OGD bound).}
      For any comparator sequence $\{u_t\}\subset A$ with path length
      $P_T=\sum_{t=2}^T|u_t-u_{t-1}|$, projected OGD with constant
      step size $\eta=Q_{\max}/\sqrt{T(1+P_T)}$ satisfies
      \[
        \sum_{t=1}^T\psi_t(q_t)-\sum_{t=1}^T\psi_t(u_t)
        \;\le\; \frac{Q_{\max}^2}{2\eta}+\frac{\eta}{2}\sum_{t=1}^T
        \|\tilde{g}_t\|^2 + Q_{\max}P_T
        = O\!\bigl(\sqrt{T(1+P_T)}\bigr),
      \]
      using $\|\tilde{g}_t\|\le\max(\alpha,1-\alpha)\le 1$ and
      $Q_{\max}=O(1)$ (see e.g.~\cite{jadbabaie2015}, Theorem 1).
\item \textbf{(Coverage and efficiency bounds).}
      With comparator $u_t=r_t$ (for which $\psi_t(r_t)=0$):
      \[
        Q(T)=O\!\bigl(\sqrt{T(1+P_T)}\bigr),\quad
        R(T)=O\!\bigl(L\sqrt{T(1+P_T)}\bigr).
      \]
\end{enumerate}
\end{theorem}

\begin{proof}
\textbf{Part (i): Subgradient identification.}
The subdifferential of $\psi_t$ at $q$ is
\[
\partial\psi_t(q)=\begin{cases}
\{-(1-\alpha)\}&q<r_t,\\
[-(1-\alpha),\alpha]&q=r_t,\\
\{\alpha\}&q>r_t.
\end{cases}
\]
Define $\tilde{g}_t:=-((1-z_t)-\alpha)$. We verify case by case:
\begin{itemize}
\item $q_t<r_t$: then $z_t=0$ (not covered), so
      $\tilde{g}_t=-(1-\alpha)\in\partial\psi_t(q_t)$. \checkmark
\item $q_t>r_t$: then $z_t=1$ (covered), so
      $\tilde{g}_t=\alpha\in\partial\psi_t(q_t)$. \checkmark
\item $q_t=r_t$: then $z_t=1$, so $\tilde{g}_t=\alpha$.
      Since $\alpha\in[-(1-\alpha),\alpha]=\partial\psi_t(r_t)$. \checkmark
\end{itemize}
Thus $q_{t+1}=\Pi_A[q_t-\eta\tilde{g}_t]$ is OGD with subgradient
$\tilde{g}_t$.

\textbf{Part (ii): Verification of OGD assumptions.}
We check all hypotheses of the dynamic OGD theorem \cite{jadbabaie2015}:
\begin{itemize}
\item \emph{Convexity of losses.} $\psi_t$ is convex (piecewise linear
      with non-decreasing slopes $-(1-\alpha)$ and $\alpha$). \checkmark
\item \emph{Bounded domain.} $A=[0,Q_{\max}]$ is compact and convex.
      Diameter $Q_{\max}<\infty$. \checkmark
\item \emph{Bounded subgradients.}
      $|\tilde{g}_t|\le\max(\alpha,1-\alpha)\le 1$. \checkmark
\item \emph{Admissible comparator.} $u_t=r_t\in A$ for all $t$. \checkmark
\end{itemize}
The dynamic OGD bound with constant step size $\eta$ gives
\[
\sum_t\psi_t(q_t)-\sum_t\psi_t(u_t)
\le \frac{Q_{\max}^2}{2\eta}+\frac{\eta}{2}T
    +\frac{Q_{\max}P_T}{\eta}\cdot\eta
= \frac{Q_{\max}^2}{2\eta}+\frac{\eta T}{2}+Q_{\max}P_T.
\]
Choosing $\eta=Q_{\max}/\sqrt{T}$ gives $O(Q_{\max}\sqrt{T}+Q_{\max}P_T)
=O(\sqrt{T(1+P_T)})$ (absorbing $Q_{\max}=O(1)$).

\textbf{Part (iii): Translating pinball regret to $Q(T)$ and $R(T)$.}

\emph{Coverage.} With $u_t=r_t$ and $\psi_t(r_t)=0$,
part (ii) gives $\sum_t\psi_t(q_t)=O(\sqrt{T(1+P_T)})$.
From the pinball definition:
$\psi_t(q)\ge(1-\alpha)(r_t-q)_+$, so
$(r_t-q_t)_+\le\psi_t(q_t)/(1-\alpha)$.
Summing: $Q(T)\le\frac{1}{1-\alpha}\sum_t\psi_t(q_t)=
O(\sqrt{T(1+P_T)})$.

\emph{Efficiency.} Since $r_t=\arg\min_{q\ge r_t}f_t(q)$ by
monotonicity of $f_t$, for any $q_t$:
$f_t(q_t)-f_t(r_t)\le L|q_t-r_t|$.
From the pinball: $|q-r_t|\le\frac{1}{\min(\alpha,1-\alpha)}\psi_t(q)$
(using $(r_t-q)_+\le\frac{1}{1-\alpha}\psi_t(q)$ and
$(q-r_t)_+\le\frac{1}{\alpha}\psi_t(q)$).
So $R(T)\le\frac{L}{\min(\alpha,1-\alpha)}\sum_t\psi_t(q_t)
=O(L\sqrt{T(1+P_T)})$.
\end{proof}

\begin{remark}[What this says about ACI]
The standard ACI guarantee \cite{gibbs2021} controls the signed average
$\frac{1}{T}\sum_t(z_t-\alpha)\to 0$. Our Theorem~\ref{thm:adversarial}
gives a \emph{strictly stronger} bound (absolute, per-term, for both
coverage and efficiency) at the same algorithmic cost---because it
measures performance against the dynamic comparator $r_t$, whereas the
ACI bound uses a fixed $\alpha$ target that allows positive and negative
errors to cancel.
\end{remark}

%==================================================================
\section{Model II: Stochastic Scalar Scores, Full Feedback}
\label{sec:scalar}
%==================================================================

\paragraph{Transition from Model~I.}
Model I required no distributional structure but the adversarial rate
$O(\sqrt{T})$ is far from what is achievable when scores are stochastic.
Here we impose a stochastic model---scores are independent draws from
a time-varying distribution---and gain two things: a much better rate
$T^{2/3}$ rather than $T^{1/2}$, and a matching \emph{lower bound}
showing $T^{2/3}$ is unavoidable. The learner still observes the full
score $s_t$ (not just the coverage bit), which is the key feature that
makes $T^{2/3}$ achievable; Section~\ref{sec:conditional} will show that
restricting to a single bit raises the rate to $T^{5/6}$.

\subsection{Setup}

We now work in the scalar setting: no covariates ($d=0$), one global
threshold $q_t\in A=[0,1]$. Scores $s_t\sim F_t$ are drawn
independently.

\begin{definition}[Performance metrics, scalar stochastic]
\label{def:scalar-metrics}
\[
R(T)=\sum_{t=1}^T\E|q_t-q_t^*|,\quad
Q(T)=\sum_{t=1}^T\E|F_t(q_t)-(1-\alpha)|,
\]
where $q_t^*=F_t^{-1}(1-\alpha)$ is the oracle threshold.
Both use absolute values: positive and negative errors cannot cancel.
\end{definition}

\begin{definition}[CDF-variation budget]
\label{def:vt}
\[
V_T=\sum_{t=1}^{T-1}\sup_{q\in A}|F_{t+1}(q)-F_t(q)|.
\]
This measures how much the score distribution drifts in $\ell^\infty$
(CDF-supremum) distance per step.
\end{definition}

\paragraph{Assumptions.}
\begin{assumption}\label{ass:scalar}
\begin{enumerate}[label=(A\arabic*)]
\item \textbf{Independence.} Scores $s_t$ are independent across $t$,
      with $s_t\sim F_t$.
\item \textbf{Density lower bound.} There exists $f_{\min}>0$ such that
      $f_t(q):=F_t'(q)\ge f_{\min}$ for all $q\in A=[0,1]$, $t\ge 1$.
      This ensures $F_t$ is strictly increasing, so $q_t^*$ is uniquely
      defined and the inverse map is $f_{\min}$-Lipschitz.
\item \textbf{Uniform concentration.} There exists $C_{VC}>0$ such that
      for every $W\ge 1$ and $t>W$,
      \[
        \E\!\left[\sup_{q\in A}
        \left|\widehat{F}_{t-1,W}(q)-\bar{F}_{t-1,W}(q)\right|\right]
        \le\frac{C_{VC}}{\sqrt{W}},
      \]
      where $\widehat{F}_{t-1,W}(q)=\frac{1}{W}\sum_{\tau=t-W}^{t-1}
      \mathbf{1}(s_\tau\le q)$ is the empirical CDF and
      $\bar{F}_{t-1,W}(q)=\frac{1}{W}\sum_{\tau=t-W}^{t-1}F_\tau(q)$
      is its expectation.
\end{enumerate}
\end{assumption}

\begin{remark}[Status of Assumption A3]
\label{rem:dkw}
Assumption A3 follows from the \textbf{Dvoretzky--Kiefer--Wolfowitz
(DKW) inequality} \cite{massart1990} and does not need to be assumed
separately. Specifically, for each $\tau$, $\mathbf{1}(s_\tau\le q)$
is a Bernoulli random variable with mean $F_\tau(q)$; since scores are
independent across $\tau$ (Assumption A1), the window
$\{s_{t-W},\dots,s_{t-1}\}$ consists of $W$ \emph{independent} (but
not identically distributed) observations. The DKW inequality for
i.n.i.d.\ (independent non-identically distributed) samples gives
\[
  \E\!\left[\sup_q|\widehat{F}_{t-1,W}(q)-\bar{F}_{t-1,W}(q)|\right]
  \le\sqrt{\frac{\pi}{2W}},
\]
so Assumption A3 holds with $C_{VC}=\sqrt{\pi/2}$. We retain A3 as a
formal assumption to make the constant explicit and to allow tighter
bounds from other concentration tools if desired.
\end{remark}

\subsection{Algorithm: Sliding-Window Empirical Quantile}

\paragraph{Initialization.} For $t=1,\dots,W$, play any $q_t\in A$
and observe $s_t$. These rounds pay at most $W$ to the total error.

\paragraph{Update.} For every $t>W$:
\begin{enumerate}[label=(\arabic*)]
\item Build the sliding-window empirical CDF:
      $\widehat{F}_{t-1,W}(q)=\frac{1}{W}\sum_{\tau=t-W}^{t-1}
      \mathbf{1}(s_\tau\le q)$.
\item Set $q_t=\inf\{q\in A:\widehat{F}_{t-1,W}(q)\ge 1-\alpha\}$.
\item Play $q_t$, observe $s_t$.
\end{enumerate}

\paragraph{Intuition.}
The algorithm maintains a window of the $W$ most recent scores and
plays the empirical $(1-\alpha)$-quantile of that window. A large $W$
gives a better estimate of the current CDF but reacts slowly to
distribution shift; a small $W$ reacts quickly but has high variance.
The optimal $W^*$ balances these effects and depends on $V_T$.

\subsection{Upper Bound}

\begin{theorem}[Scalar stochastic upper bound]
\label{thm:scalar-upper}
Under Assumption~\ref{ass:scalar}, with window size
\[
W^*=\min\!\left\{\!\left\lceil\!\left(\frac{C_{VC}}{2}\right)^{\!2/3}
\!\!\left(\frac{T}{V_T}\right)^{\!2/3}\right\rceil, T\right\},
\]
the sliding-window algorithm satisfies
\begin{align*}
R(T)&=O\!\left(\!\left(\frac{T}{V_T}\right)^{\!2/3}
          +\frac{T^{2/3}V_T^{1/3}}{f_{\min}}\right),\\
Q(T)&=O\!\left(\!\left(\frac{T}{V_T}\right)^{\!2/3}
          +T^{2/3}V_T^{1/3}\right).
\end{align*}
\end{theorem}

\subsection{Proof of Theorem~\ref{thm:scalar-upper}}

The proof decomposes the total error into three sources---estimation
noise in the empirical CDF, bias from distribution drift within the
window, and the discrete jump size of the empirical CDF---bounds each,
then balances the window size $W$ to minimize the sum.

\subsubsection{Step 1: Uniform Concentration}

Define the empirical process deviation at time $t$:
\[
\Delta_{t,W}:=\sup_{q\in A}|\widehat{F}_{t-1,W}(q)-\bar{F}_{t-1,W}(q)|.
\]
By Assumption A3:
\begin{equation}\label{eq:concentration}
\E[\Delta_{t,W}]\le\frac{C_{VC}}{\sqrt{W}}.
\end{equation}

\subsubsection{Step 2: Quantile-Crossing Lemma}

\begin{lemma}[Quantile-crossing lemma]
\label{lem:qcl}
Define the window-to-current drift
$\mathcal{E}_t:=\sup_q|\bar{F}_{t-1,W}(q)-F_t(q)|$.
For any $t>W$, the algorithm's choice $q_t$ satisfies
\[
|F_t(q_t)-(1-\alpha)|\le\Delta_{t,W}+\mathcal{E}_t+\frac{1}{W}.
\]
\end{lemma}

\begin{proof}
We establish a lower and upper bound on $F_t(q_t)$ separately.

\emph{Lower bound.}
By the infimum definition of $q_t$, the empirical CDF satisfies
$\widehat{F}_{t-1,W}(q_t)\ge 1-\alpha$ (right-continuity of the
empirical CDF ensures the infimum is attained). Therefore:
\[
\bar{F}_{t-1,W}(q_t)\ge\widehat{F}_{t-1,W}(q_t)-\Delta_{t,W}
\ge (1-\alpha)-\Delta_{t,W}.
\]
Then, since $|\bar{F}_{t-1,W}(q_t)-F_t(q_t)|\le\mathcal{E}_t$:
\[
F_t(q_t)\ge\bar{F}_{t-1,W}(q_t)-\mathcal{E}_t
\ge(1-\alpha)-\Delta_{t,W}-\mathcal{E}_t.
\]

\emph{Upper bound.}
Since $\widehat{F}_{t-1,W}$ is a step function with jump size exactly
$1/W$, the point just to the left of $q_t$ satisfies
$\widehat{F}_{t-1,W}(q_t^-)<1-\alpha$ (otherwise $q_t$ would not be
the infimum). Therefore the value at $q_t$ overshoots $1-\alpha$ by
at most one jump:
\[
\widehat{F}_{t-1,W}(q_t)\le(1-\alpha)+\frac{1}{W}.
\]
Chaining: $\bar{F}_{t-1,W}(q_t)\le\widehat{F}_{t-1,W}(q_t)+\Delta_{t,W}
\le(1-\alpha)+\Delta_{t,W}+\frac{1}{W}$, and
\[
F_t(q_t)\le\bar{F}_{t-1,W}(q_t)+\mathcal{E}_t
\le(1-\alpha)+\Delta_{t,W}+\mathcal{E}_t+\frac{1}{W}.
\]
Combining the two bounds gives the lemma.
\end{proof}

\subsubsection{Step 3: Converting to Threshold-Space Error}

By Assumption A2, $F_t$ has density $\ge f_{\min}$. By the Mean Value
Theorem applied to $F_t$ between $q_t$ and $q_t^*$, there exists
$\tilde{q}$ between them with
$|F_t(q_t)-F_t(q_t^*)|=f_t(\tilde{q})|q_t-q_t^*|\ge f_{\min}|q_t-q_t^*|$.
Since $F_t(q_t^*)=1-\alpha$:
\[
|q_t-q_t^*|\le\frac{|F_t(q_t)-(1-\alpha)|}{f_{\min}}.
\]
Taking expectations and applying Lemma~\ref{lem:qcl} and
\eqref{eq:concentration}:
\begin{equation}\label{eq:action-bound}
\E|q_t-q_t^*|\le\frac{1}{f_{\min}}\!\left(
  \frac{C_{VC}}{\sqrt{W}}+\mathcal{E}_t+\frac{1}{W}\right).
\end{equation}

\subsubsection{Step 4: Drift Telescoping}

\begin{lemma}[Cumulative drift bound]
\label{lem:drift}
$\displaystyle\sum_{t=W+1}^T\mathcal{E}_t\le W\cdot V_T.$
\end{lemma}

\begin{proof}
Fix $t>W$. For any $\tau\in[t-W,t-1]$ and $q\in A$, telescoping gives
\[
|F_\tau(q)-F_t(q)|\le\sum_{k=\tau}^{t-1}\sup_{q'}|F_{k+1}(q')-F_k(q')|.
\]
Averaging over $\tau\in[t-W,t-1]$:
\[
\mathcal{E}_t=\sup_q\left|\frac{1}{W}\sum_{\tau=t-W}^{t-1}(F_\tau(q)-F_t(q))\right|
\le\frac{1}{W}\sum_{\tau=t-W}^{t-1}\sum_{k=\tau}^{t-1}\sup_{q'}|F_{k+1}(q')-F_k(q')|.
\]
Summing over $t=W+1$ to $T$ and exchanging order of summation: each
index $k\in\{1,\dots,T-1\}$ appears in the inner sum for at most $W$
values of $t$, so
\[
\sum_{t=W+1}^T\mathcal{E}_t\le W\sum_{k=1}^{T-1}\sup_{q'}|F_{k+1}(q')-F_k(q')|
=W\cdot V_T.\qedhere
\]
\end{proof}

\subsubsection{Step 5: Assembling and Balancing}

\emph{Absolute calibration error $Q(T)$.}
For the first $W$ rounds, $|F_t(q_t)-(1-\alpha)|\le 1$.
For $t>W$, Lemma~\ref{lem:qcl} and \eqref{eq:concentration} give:
\[
Q(T)\le W+\sum_{t=W+1}^T\!\left(\frac{C_{VC}}{\sqrt{W}}+\mathcal{E}_t
+\frac{1}{W}\right)
\le W+\frac{C_{VC}T}{\sqrt{W}}+WV_T+\frac{T}{W}.
\]

\emph{Tracking error $R(T)$.}
Analogously from \eqref{eq:action-bound}:
$R(T)\le W+\frac{1}{f_{\min}}\!\left(\frac{C_{VC}T}{\sqrt{W}}
+WV_T+\frac{T}{W}\right)$.

\emph{Balancing $W$.}
Consider the dominant terms $h(W)=\frac{C_{VC}T}{\sqrt{W}}+V_TW$.
Setting $h'(W)=0$:
\[
-\frac{C_{VC}T}{2W^{3/2}}+V_T=0\implies
W^*=\left(\frac{C_{VC}}{2}\right)^{2/3}\!\!\left(\frac{T}{V_T}\right)^{2/3}.
\]
At $W=\lceil W^*\rceil$: $h(W^*)=\frac{3}{2}\left(\frac{C_{VC}}{2}\right)^{2/3}
T^{2/3}V_T^{1/3}$.

The residual term $T/W^*\asymp T^{1/3}V_T^{2/3}=T^{2/3}V_T^{1/3}(V_T/T)^{1/3}
\le T^{2/3}V_T^{1/3}$ (using $V_T\le T$), so it is lower order.
The initialization term $W^*\asymp(T/V_T)^{2/3}$. Combining:
\[
Q(T)=O\!\left(\!\left(\frac{T}{V_T}\right)^{\!2/3}\!+T^{2/3}V_T^{1/3}\right),
\quad
R(T)=O\!\left(\!\left(\frac{T}{V_T}\right)^{\!2/3}
+\frac{T^{2/3}V_T^{1/3}}{f_{\min}}\right).\qquad\blacksquare
\]

\subsection{Minimax Lower Bound}

\paragraph{The fundamental identification problem.}
Before stating the lower bound, it helps to identify the core
statistical challenge. An algorithm choosing $q_t$ at each round faces
an \emph{estimation problem}: it must distinguish the current oracle
threshold $q_t^*=F_t^{-1}(1-\alpha)$ from a nearby alternative, using
only a finite window of past scores. The key difficulty is that
\emph{any two distributions that are close in KL divergence require many
samples to tell apart}, yet the oracle threshold can change between
them. The lower bound formalizes this by constructing a two-distribution
``hypothesis testing'' problem where: the oracle thresholds differ by
$\Delta$, but the distributions are so similar that $B\sim 1/\Delta^2$
samples are needed to distinguish them. During these $B$ rounds the
algorithm is essentially guessing, paying at least $\Delta/2$ in
tracking error per round. Summing over $K=T/B$ blocks gives the
$\Omega(T\Delta)$ lower bound, and optimizing $\Delta$ against $V_T$
yields $T^{2/3}V_T^{1/3}$.

\begin{theorem}[Minimax lower bound]
\label{thm:scalar-lower}
For every online algorithm $\mathcal{A}$ and sufficiently small
universal constant $c_2>0$, for any $V_T\le c_2 T$:
\[
\inf_{\mathcal{A}}\sup_{\{F_t\}\in\mathcal{F}(V_T)}R(T)\ge c_1T^{2/3}V_T^{1/3},
\quad
\inf_{\mathcal{A}}\sup_{\{F_t\}\in\mathcal{F}(V_T)}Q(T)\ge c_1f_{\min}T^{2/3}V_T^{1/3},
\]
where $c_1>0$ is a universal constant.
\end{theorem}

\begin{proof}
The proof proceeds in four steps: (1) construct two hard distributions,
(2) bound the sample complexity of distinguishing them, (3) embed the
testing problem into the tracking problem via a block structure, and
(4) verify the resulting distribution sequence is within $\mathcal{F}(V_T)$.

\textbf{Step 1: Two-distribution construction.}
Fix $\alpha\in(0,1)$ and a small perturbation $\varepsilon\in(0,\alpha)$.
Let $P_0$ be uniform on $[0,1]$ (density $f_0\equiv 1$, oracle quantile
$q_0^*=1-\alpha$). Let $P_1$ have piecewise-constant density
\[
f_1(q)=\begin{cases}1+\varepsilon&q\in[0,1-\alpha],\\
1-\frac{(1-\alpha)\varepsilon}{\alpha}&q\in(1-\alpha,1].\end{cases}
\]
Note $f_1$ integrates to $1$ and is a valid density for $\varepsilon<\alpha$.
The oracle quantile for $P_1$ solves $(1+\varepsilon)q_1^*=1-\alpha$,
giving $q_1^*=\frac{1-\alpha}{1+\varepsilon}$.
The separation is $\Delta:=q_0^*-q_1^*=\frac{(1-\alpha)\varepsilon}{1+\varepsilon}
=\Theta(\varepsilon)$.

The KL divergence (Taylor expanding to second order in $\varepsilon$):
\[
\dkl{P_0}{P_1}=(1-\alpha)\log\frac{1}{1+\varepsilon}+\alpha\log\frac{1}{1-\frac{(1-\alpha)\varepsilon}{\alpha}}
=\frac{(1-\alpha)\varepsilon^2}{2\alpha}+O(\varepsilon^3)\le C\Delta^2,
\]
for a constant $C=\frac{1-\alpha}{2\alpha(1-\alpha)^2}\cdot(1+o(1))$
(using $\varepsilon=\Theta(\Delta)$).

\textbf{Step 2: Sample complexity of testing.}
Divide the horizon $T$ into $K$ blocks of length $B=\lfloor T/K\rfloor$.
For block $k$, the adversary independently draws $\Theta_k\in\{0,1\}$
uniformly at random (unknown to the learner) and generates all $B$
scores in that block i.i.d.\ from $P_{\Theta_k}$.

Consider any round $t$ in block $k$. The learner's threshold
$q_t$ depends on all past scores $(s_1,\dots,s_{t-1})$ and
internal randomness $U$.
Let $\mathcal{H}_{k-1}$ be the $\sigma$-algebra of all information
before block $k$ begins. By construction, $\Theta_k$ is independent
of $\mathcal{H}_{k-1}$ and $U$.

\emph{The decoder.}
We use $q_t$ to construct a guess for $\Theta_k$. Define:
\[
\phi_t:=\mathbf{1}\!\left\{|q_t-q_1^*|<|q_t-q_0^*|\right\}.
\]
In words: $\phi_t=1$ if the learner's threshold is closer to $q_1^*$
than to $q_0^*$, and $\phi_t=0$ otherwise. This is the natural
``nearest-neighbour'' decoder for the two-point hypothesis test.
If $\phi_t\ne\Theta_k$, then $q_t$ is on the wrong side of the midpoint
$(q_0^*+q_1^*)/2$, which implies
\[
|q_t-q_{\Theta_k}^*|\ge\frac{\Delta}{2}.
\]
(When $\Theta_k=0$ and $\phi_t=1$: $q_t$ is closer to $q_1^*$, so
$|q_t-q_0^*|>|q_t-q_1^*|\ge 0$, and by the midpoint argument
$|q_t-q_0^*|\ge\Delta/2$. Symmetric for $\Theta_k=1$.)

\emph{Bounding the error probability.}
Conditional on $(\mathcal{H}_{k-1},U)=(h,u)$, the decoder $\phi_t$ is
a deterministic measurable function of the current block's $B$ scores,
which are i.i.d.\ from $P_{\Theta_k}$. Le Cam's lemma applied to this
conditional binary testing problem gives:
\[
\Prob(\phi_t\ne\Theta_k|\mathcal{H}_{k-1}=h,U=u)
\ge\frac{1}{2}\bigl(1-\tv{P_0^B,P_1^B}\bigr).
\]
By Pinsker's inequality and tensorization of KL divergence:
\[
\tv{P_0^B,P_1^B}
\le\sqrt{\tfrac{1}{2}\dkl{P_0^B}{P_1^B}}
=\sqrt{\tfrac{B}{2}\dkl{P_0}{P_1}}
\le\sqrt{\tfrac{BC\Delta^2}{2}}.
\]
Choosing $B=\lfloor\frac{1}{8C\Delta^2}\rfloor$ ensures
$\tv{P_0^B,P_1^B}\le\frac{1}{4}$, so $\Prob(\phi_t\ne\Theta_k|\mathcal{H}_{k-1},U)\ge\frac{3}{8}$.
Taking unconditional expectation: $\Prob(\phi_t\ne\Theta_k)\ge\frac{3}{8}$.

\textbf{Step 3: Lower bounding the tracking error.}
Summing over all $B$ rounds in block $k$:
\[
\sum_{t\in\text{block }k}\E|q_t-q_{\Theta_k}^*|
\ge\frac{\Delta}{2}\sum_{t\in\text{block }k}\Prob(\phi_t\ne\Theta_k)
\ge\frac{3\Delta B}{8}.
\]
Summing over $K=T/B$ blocks: $R(T)\ge\frac{3\Delta}{8}\cdot KB
=\frac{3T\Delta}{8}=\Omega(T\Delta)$.

By a standard averaging argument: if the expected tracking error over
the random block labels is $\ge c_3 T\Delta$, then there exists at least
one deterministic realization of block labels giving error $\ge c_3T\Delta$.
Fix that realization to get a specific CDF sequence $\{F_t^{\mathcal{A}}\}$
(which may depend on the algorithm, hence the superscript) with
$R(T;\mathcal{A},\{F_t^{\mathcal{A}}\})\ge c_3T\Delta$.

\textbf{Step 4: Verifying the variation budget.}
The constructed sequence $\{F_t^{\mathcal{A}}\}$ changes CDF only at
block boundaries where $\Theta_k$ changes. At each such switch,
$\sup_q|F_0(q)-F_1(q)|=(1-\alpha)\varepsilon=(1+\varepsilon)\Delta$.
The number of switches is at most $K$. Therefore:
\[
V_{\rm seq}\le K(1+\varepsilon)\Delta=\frac{T}{B}(1+\varepsilon)\Delta.
\]
For sufficiently small $\Delta$, $B\ge\frac{1}{16C\Delta^2}$
(using the floor bound $B\ge\frac{1}{8C\Delta^2}-1$), so:
\[
V_{\rm seq}\le 16CT\Delta^3(1+\varepsilon)\le C'T\Delta^3,
\]
where $C'>0$ absorbs the $(1+\varepsilon)$ factor (valid for $\varepsilon$
small, i.e.\ $\Delta$ small).

\emph{Choosing $\Delta$ to match $V_T$.}
Set $\Delta=c_0(V_T/T)^{1/3}$ for small $c_0>0$.
Then $V_{\rm seq}\le C'c_0^3V_T\le V_T$ for $c_0\le(1/C')^{1/3}$.
The tracking lower bound becomes:
\[
R(T)\ge c_3T\Delta=c_3c_0T^{2/3}V_T^{1/3}=:c_1T^{2/3}V_T^{1/3}.
\]
This holds for $V_T\le c_2T$ where $c_2>0$ ensures $\varepsilon<\alpha$
(a constraint from the density construction). Since
$\{F_t^{\mathcal{A}}\}\in\mathcal{F}(V_T)$ and this holds for every
algorithm $\mathcal{A}$, the infimum over algorithms satisfies the bound.

\emph{Bound for $Q(T)$.}
The geometric coupling (MVT, density bounded below by $f_{\min}$):
$|F_t(q_t)-(1-\alpha)|\ge f_{\min}|q_t-q_t^*|$. Summing:
$Q(T)\ge f_{\min}R(T)\ge c_1f_{\min}T^{2/3}V_T^{1/3}$.
\end{proof}

\begin{corollary}[Minimax optimality]
\label{cor:scalar-optimal}
The sliding-window algorithm is asymptotically minimax optimal:
\[
\Omega\bigl(T^{2/3}V_T^{1/3}\bigr)
\le\inf_{\mathcal{A}}\sup_{\{F_t\}\in\mathcal{F}(V_T)}R(T)
\le O\!\left(\!\left(\frac{T}{V_T}\right)^{\!2/3}+T^{2/3}V_T^{1/3}\right).
\]
The initialization term $(T/V_T)^{2/3}$ is dominated by $T^{2/3}V_T^{1/3}$
whenever $V_T\to\infty$.
\end{corollary}

%==================================================================
\section{Model III: Stochastic Conditional Scores, Single-Bit Feedback}
\label{sec:conditional}
%==================================================================

\paragraph{Transition from Model~II.}
Model II achieved the optimal $T^{2/3}$ rate by exploiting full score
feedback: the learner sees $s_t$, which allows constructing an empirical
CDF and querying it at any threshold. Two natural extensions make the
problem harder simultaneously: (a) restricting feedback to the single
binary bit $z_t=\mathbf{1}(s_t\le q_t)$, and (b) allowing the oracle
threshold to depend on the covariate $X_t$, requiring a function-valued
threshold $q_t:\X\to\R$ rather than a scalar. We show that these two
changes together raise the rate from $T^{2/3}$ to $T^{5/6}$ (in $d=0$)
and introduce an additional curse of dimensionality factor.

The variation budget in this section uses the \textbf{oracle path
length in threshold space}:
\[
P_T:=\sum_{t=1}^{T-1}\sup_{x\in\X}|q_{t+1}^*(x)-q_t^*(x)|
\]
rather than the CDF $\ell^\infty$-variation used in Section~\ref{sec:scalar}.
We rename to $P_T$ (matching Section~\ref{sec:adversarial}'s path-length
notation) to emphasize this difference. The two budgets are related by
$P_T\le V_T/f_{\min}$ (via the MVT applied to $F_t^{-1}$), so $P_T$ is
generally smaller and reflects more directly how much the actual
threshold target moves.

\subsection{Setup}

Fix a conformity score function $s:\X\times\Y\to\R$, held fixed
throughout. At each round $t$:
\begin{enumerate}[label=(\arabic*)]
\item Nature draws $(X_t,Y_t)\sim P_t$ (unknown, time-varying).
\item Learner observes $X_t$ and selects a threshold function
      $q_t:\X\to A$, playing $q_t(X_t)$.
\item Learner predicts $C_t(x)=\{y:s(x,y)\le q_t(x)\}$.
\item Nature reveals $Y_t$; learner observes
      $z_t=\mathbf{1}(s(X_t,Y_t)\le q_t(X_t))$ \emph{only}---no score
      value, no delayed label.
\end{enumerate}

\begin{definition}[Conditional oracle and metrics]
\label{def:cond-metrics}
\[
q_t^*(x):=F_t^{-1}(1-\alpha|x),\quad
F_t(q|x):=\Prob_t\!\bigl(s(X_t,Y_t)\le q\mid X_t=x\bigr).
\]
The prediction set size is $\mu(q,x):=\lambda(\{y:s(x,y)\le q\})$
(nondecreasing in $q$, independent of $t$, not necessarily convex).
\[
V_c(T)=\sum_{t=1}^T\E\!\bigl[(1-\alpha-F_t(q_t(X_t)|X_t))_+\bigr],\quad
R(T)=\sum_{t=1}^T\E\!\bigl[\mu(q_t(X_t),X_t)-\mu(q_t^*(X_t),X_t)\bigr].
\]
\end{definition}

\subsection{Assumptions}

\begin{assumption}[Conditional setting]
\label{ass:conditional}
\begin{enumerate}[label=(C\arabic*)]
\item \textbf{H\"{o}lder oracle.}
      $q_t^*\in\mathcal{Q}_\beta(L)=\{q:\X\to A:|q(x)-q(x')|\le L\|x-x'\|^\beta\}$
      for fixed $\beta\in(0,1]$, $L>0$, every $t$. This says the
      optimal threshold varies smoothly in covariate space.
\item \textbf{Spatial score continuity.}
      $|F_t(q|x)-F_t(q|x')|\le L_x\|x-x'\|^\beta$ uniformly in $q,t$.
\item \textbf{Oracle path-length budget.}
      $P_T:=\sum_{t=1}^{T-1}\sup_x|q_{t+1}^*(x)-q_t^*(x)|<\infty$.
\item \textbf{Independence and density bounds.}
      $(X_t,Y_t)$ independent across $t$;
      $p_t(x)\in[p_{\min},p_{\max}]$;
      conditional score density $p_t(q|x)\in[p_{\min}^s,p_{\max}^s]$
      for all $q\in A$, $t$, $x$.
      The global density floor $p_{\min}^s>0$ (over all of $A$)
      is needed for iterate confinement (see Remark~\ref{rem:confinement}).
\item \textbf{Step-size bound.}
      $\eta\le p_{\min}^s/(2(p_{\max}^s)^2)$. This ensures the
      contraction coefficient is in $[0,1)$ at every step, preventing
      the iterate from oscillating past the oracle.
\item \textbf{Lipschitz set size.}
      $|\mu(q,x)-\mu(q',x)|\le L_\mu|q-q'|$ uniformly in $x$.
      Equivalently, $\partial_q\mu\le L_\mu$ (bounded score density).
      Convexity of $\mu$ is \emph{not} assumed.
\end{enumerate}
\end{assumption}

\begin{remark}[Why global density floor is needed]
\label{rem:confinement}
The local density bound in Assumption C4 ($p_{\min}^s>0$ globally,
not just near $q_t^*$) is genuinely necessary---not a convenience.
Without it, if the iterate $u_t^j$ wanders outside the neighborhood of
$q_t^*$, the ACI update has no restoring force to bring it back, since
the MVT contraction argument relies on $p_t(\xi|x)\ge p_{\min}^s$ for
$\xi$ between the iterate and the oracle. Once outside the neighborhood,
$\xi$ may be in a region where the density is zero, and the recursion
can diverge. The global floor $p_{\min}^s>0$ (which may be much smaller
than the local density in the interesting region) ensures a
weak-but-universal restoring force everywhere. Its magnitude affects
only the burn-in time (lower order), not the final rate.
\end{remark}

\subsection{Algorithm: H\"{o}lder-Partitioned ACI (HP-ACI)}

\paragraph{Key idea.}
Because the oracle threshold $q_t^*(x)$ varies with $x$, a single
scalar ACI instance cannot track it everywhere simultaneously. We
partition the covariate space $\X=[0,1]^d$ into cells of side $h$ and
run one independent ACI instance per cell, updated only when $X_t$
falls in that cell. Cells that are visited rarely get fewer updates
but also incur less coverage error from drift; the bandwidth $h$
balances estimation (small cell = few visits = noisy update) against
approximation (large cell = coarse discretization = spatial bias).

\paragraph{Setup.}
Cover $\X$ by $N=\lceil h^{-d}\rceil$ axis-aligned cells
$\{B_j\}_{j=1}^N$ of side $h$, with reference point $x_j\in B_j$.
Maintain threshold $u_t^j\in A$ per cell.

\paragraph{Update.}
At round $t$, let $j=j(t)$ be the cell containing $X_t$:
\[
u_{t+1}^{j(t)}=\Pi_A\!\Bigl[u_t^{j(t)}+\eta\bigl((1-z_t)-\alpha\bigr)\Bigr],
\quad u_{t+1}^{j'}=u_t^{j'}\;\;\forall j'\ne j(t).
\]
The update direction $(1-z_t)-\alpha$ has conditional mean
$F_t(u_t^{j(t)}|X_t)-(1-\alpha)$ given $u_t^{j(t)}$ and $X_t$, which
is zero exactly at $q_t^*(X_t)$. This is a Robbins-Monro stochastic
approximation step toward the root $q_t^*(X_t)$.

\subsection{Main Result}

\begin{theorem}[Conditional tracking bound]
\label{thm:conditional}
Under Assumption~\ref{ass:conditional}, with
$h^*=T^{-1/(6\beta+d)}P_T^{2/(6\beta+d)}$ and per-cell step size
$\eta_j^*=(2(P_T^j)^2/(m_j p_{\min}^s))^{1/3}$ (where $P_T^j$ is
the per-cell oracle path length and $m_j$ is the expected number of
visits), HP-ACI satisfies
\[
V_c(T)=O\!\left(T^{\frac{5\beta+d}{6\beta+d}}\,P_T^{\frac{2\beta}{6\beta+d}}\right),
\quad
R(T)=O\!\left(\frac{L_\mu}{p_{\min}^s}\,
  T^{\frac{5\beta+d}{6\beta+d}}\,P_T^{\frac{2\beta}{6\beta+d}}\right).
\]
\end{theorem}

\begin{remark}[Special cases]
\begin{itemize}
\item $d=0$, $\beta=1$: $V_c(T)=O(T^{5/6}P_T^{1/3})$ under single-bit
      feedback, versus $O(T^{2/3}V_T^{1/3})$ under full-score feedback.
      The gap $T^{2/3}\to T^{5/6}$ is the cost of bandit feedback.
\item As $d\to\infty$ (relative to $\beta$), the exponent on $T$
      approaches $1$ (vacuous), the curse of dimensionality.
\item $d=0$: HP-ACI with a single cell reduces to scalar ACI.
      The signed Gibbs-Cand\`es guarantee $T^{-1}\sum_t(z_t-\alpha)\to 0$
      is weaker than our absolute $V_c(T)=O(T^{5/6}P_T^{1/3})$ bound.
\end{itemize}
\end{remark}

\subsection{Proof of Theorem~\ref{thm:conditional}}

\subsubsection{Step 1: Per-cell error recursion}

Fix cell $j$; relabel visit rounds $k=1,\dots,m$ ($m=m_j$). Let
$q_k^*=q_{t_k}^*(x_j)$ and $e_k=u_k-q_k^*$. Define
$h_k(u)=(1-F_{t_k}(u|x_j))-\alpha$, which has root at $q_k^*$
(since $F_{t_k}(q_k^*|x_j)=1-\alpha$) and slope
$h_k'(u)=-p_{t_k}(u|x_j)\le-p_{\min}^s<0$.

Decompose the update signal:
\[
(1-z_k)-\alpha=h_k(u_k)+\mathrm{noise}_k+\mathrm{bias}_k,
\]
where $\mathrm{noise}_k=(1-z_k)-(1-F_{t_k}(u_k|X_{t_k}))$ satisfies
$\E[\mathrm{noise}_k|\mathcal{H}_{k-1},X_{t_k}]=0$, $|\mathrm{noise}_k|\le 2$;
and the spatial bias $\mathrm{bias}_k=F_{t_k}(u_k|x_j)-F_{t_k}(u_k|X_{t_k})$
satisfies $|\mathrm{bias}_k|\le L_x d^{\beta/2}h^\beta$ (by Assumption C2).

By the MVT, $h_k(u_k)=-p_{t_k}(\xi_k|x_j)e_k$ for $\xi_k$ between
$u_k$ and $q_k^*$. The projection is non-expansive, giving:
\begin{equation}\label{eq:cond-recur}
|e_{k+1}|\le|e_k(1-\eta p_{t_k}(\xi_k|x_j))|+\eta|\mathrm{noise}_k|
+\eta|\mathrm{bias}_k|+|\Delta_k|,
\end{equation}
where $\Delta_k=q_{k+1}^*-q_k^*$ is the oracle drift between visits.

\subsubsection{Step 2: Lyapunov recursion}

Let $v_k=\E[e_k^2]$ and $\rho_k=1-\eta p_{t_k}(\xi_k|x_j)$.
Under Assumption C5 ($\eta\le p_{\min}^s/(2(p_{\max}^s)^2)$),
we verify $\rho_k\in[0,1)$: the upper bound $\rho_k\le 1-\eta p_{\min}^s<1$
holds since $\eta>0$; the lower bound $\rho_k\ge 0$ requires
$\eta p_{t_k}(\xi_k|x_j)\le\eta p_{\max}^s\le p_{\min}^s/(2p_{\max}^s)\le 1$.

Squaring \eqref{eq:cond-recur} and taking conditional expectation
(using $\E[\mathrm{noise}_k|\mathcal{H}_{k-1},X_{t_k}]=0$ to kill
cross-terms with the noise):
\[
\E[e_{k+1}^2|\mathcal{H}_k]
\le\rho_k^2e_k^2+\eta^2\sigma^2+\frac{\rho_k^2}{\eta p_{\min}^s}
   (\eta|\mathrm{bias}_k|+|\Delta_k|)^2+\eta p_{\min}^s e_k^2,
\]
where we applied Young's inequality $2\rho_k e_k Y\le\eta p_{\min}^s e_k^2
+\frac{\rho_k^2}{\eta p_{\min}^s}Y^2$ with $Y=\eta|\mathrm{bias}_k|+|\Delta_k|$,
and used $\sigma^2=\E[\mathrm{noise}_k^2|\mathcal{H}_k]\le 4$.

The combined coefficient on $e_k^2$ is $\rho_k^2+\eta p_{\min}^s$.
Under Assumption C5, at $\rho_k=1-\eta p_{\max}^s$ (worst case):
$\rho_k^2+\eta p_{\min}^s=(1-\eta p_{\max}^s)^2+\eta p_{\min}^s
\le 1-\eta p_{\max}^s(2-\eta p_{\max}^s)+\eta p_{\min}^s
\le 1-\eta p_{\max}^s+\frac{(\eta p_{\max}^s)^2}{p_{\min}^s/p_{\max}^s}
+\eta p_{\min}^s$.
Using $\eta p_{\max}^s\le p_{\min}^s/(2p_{\max}^s)\le 1$ and
$p_{\max}^s\ge p_{\min}^s$:
$\rho_k^2+\eta p_{\min}^s\le 1-\tfrac{1}{2}\eta p_{\min}^s$.
(Full algebra: $(1-\eta p_{\max}^s)^2+\eta p_{\min}^s
=1-2\eta p_{\max}^s+\eta^2(p_{\max}^s)^2+\eta p_{\min}^s
\le 1-\eta p_{\min}^s$ for $\eta(p_{\max}^s)^2\le p_{\min}^s/2$,
which is exactly Assumption C5.)

Setting $\gamma=\frac{1}{2}\eta p_{\min}^s$ and taking full expectation:
\begin{equation}\label{eq:cond-lyap}
v_{k+1}\le(1-2\gamma)v_k+4\eta^2
+\frac{4\eta L_x^2 d^\beta h^{2\beta}}{p_{\min}^s}
+\frac{4\Delta_k^2}{\eta p_{\min}^s}.
\end{equation}

\subsubsection{Step 3: Unrolling and step-size optimization}

By Lemma~\ref{lem:telescoping} (telescoping a geometric recursion),
applied to \eqref{eq:cond-lyap}:
\[
\sum_{k=1}^mv_k
=O\!\left(\frac{m\eta}{p_{\min}^s}+\frac{mh^{2\beta}}{(p_{\min}^s)^2}
+\frac{(P_T^j)^2}{\eta^2(p_{\min}^s)^2}\right),
\]
where $P_T^j:=\sum_k|\Delta_k|\le P_T$ (oracle path length within cell
$j$, bounded by the global path length since the supremum over $x$ is
used in $P_T$), and we used $\sum_k\Delta_k^2\le(\sum_k|\Delta_k|)^2=(P_T^j)^2$.

Minimizing over $\eta$ (balancing $m\eta$ against $(P_T^j)^2/\eta^2$):
$\eta_j^*=(2(P_T^j)^2/(mp_{\min}^s))^{1/3}$,
giving $\sum_kv_k=O(m^{2/3}(P_T^j)^{2/3}/(p_{\min}^s)^{4/3})$.

By Cauchy-Schwarz (pathwise) and Jensen (concavity of $\sqrt{\cdot}$):
\begin{equation}\label{eq:cell-bound}
\sum_{k=1}^m\E|e_k|\le\sqrt{m\sum_kv_k}
=O\!\left(\frac{m^{5/6}(P_T^j)^{1/3}}{p_{\min}^s}
+\frac{mh^\beta}{p_{\min}^s}\right).
\end{equation}

\subsubsection{Step 4: Visit concentration}

The proof uses $m_j\approx p_{\min}h^dT$ per cell. This holds in
expectation ($\E[m_j]\ge p_{\min}h^dT$) and with high probability:

\begin{lemma}[Visit concentration]\label{lem:visits}
With probability at least $1-h^{-d}\exp(-p_{\min}h^dT/8)$,
every cell has $m_j\ge p_{\min}h^dT/2$.
\end{lemma}

\begin{proof}
Each indicator $\mathbf{1}(X_t\in B_j)$ is Bernoulli with mean
$\ge p_{\min}h^d$ (by C4). These are independent across $t$ (by C4).
Chernoff's lower-tail bound: $\Prob(m_j\le\mu_j/2)\le e^{-\mu_j/8}$
with $\mu_j=\E[m_j]\ge p_{\min}h^dT$.
Union bound over $N\le h^{-d}$ cells completes the proof.
\end{proof}

Under Assumption C3/non-degeneracy ($h^dT\to\infty$ at $h=h^*$), the
failure probability is super-polynomially small and contributes $o(1)$
to the expected bounds (trivially bounding each round's contribution by
$1$ on the failure event, then multiplying by $T\cdot\text{(failure prob)}$).
Henceforth condition on the high-probability event $m_j\in[p_{\min}h^dT/2,
p_{\max}h^dT]$.

\subsubsection{Step 5: Aggregation and balancing}

\emph{Cell budget.}
For each $j$: $P_T^j\le P_T$ (using the supremum over $x$ in $P_T$).
So $\sum_j P_T^j\le NP_T=h^{-d}P_T$ and $\sum_j(P_T^j)^{1/3}\le N^{2/3}
(\sum_j P_T^j)^{1/3}$ (by H\"{o}lder) $\le h^{-2d/3}P_T^{1/3}$.
With $m_j\le p_{\max}h^dT$ on the high-probability event:
\[
\sum_j m_j^{5/6}(P_T^j)^{1/3}
\le(p_{\max}h^dT)^{5/6}\cdot h^{-2d/3}P_T^{1/3}
=O\!\left(T^{5/6}h^{-d/6}P_T^{1/3}\right).
\]
The spatial approximation term: $\sum_j m_j h^\beta\le T h^\beta$.

\emph{Total violation bound.}
Translating $\E|e_k|$ to violation via the MVT
($(1-\alpha-F_t(q_t|X_t))_+\le p_{\max}^s\E|e_k|$ plus a bias
$\le p_{\max}^s Lh^\beta$ from the spatial oracle gap):
\[
V_c(T)=O\!\left(T^{5/6}h^{-d/6}P_T^{1/3}+Th^\beta\right).
\]

\emph{Balancing.}
Set $T^{5/6}h^{-d/6}P_T^{1/3}\asymp Th^\beta$:
\[
h^{\beta+d/6}\asymp T^{-1/6}P_T^{1/3}
\implies
h^*=T^{-\frac{1}{6\beta+d}}P_T^{\frac{2}{6\beta+d}}.
\]
Then $T(h^*)^\beta=T^{(5\beta+d)/(6\beta+d)}P_T^{2\beta/(6\beta+d)}$.

\emph{Regret $R(T)$.}
By Assumption C6: $\mu(q_t(x),x)-\mu(q_t^*(x),x)\le L_\mu|q_t(x)-q_t^*(x)|$
(Lipschitz, no convexity). The same aggregation gives
$R(T)=O(L_\mu/p_{\min}^s)$ times the same rate. $\blacksquare$

\begin{lemma}[Lyapunov telescoping]\label{lem:telescoping}
If $v_{k+1}\le(1-2\gamma)v_k+C_k$ with $\gamma\in(0,1/2)$, then
$\sum_{k=1}^mv_k\le v_1/\gamma+(1/\gamma)\sum_{k=1}^mC_k$.
\end{lemma}
\begin{proof}
Rearrange: $2\gamma v_k\le v_k-v_{k+1}+C_k$.
Sum from $k=1$ to $m$: $2\gamma\sum_{k=1}^mv_k\le v_1-v_{m+1}+\sum_kC_k
\le v_1+\sum_kC_k$. Divide by $2\gamma$.
\end{proof}

%==================================================================
\section{Adaptive Step-Size Selection}
\label{sec:adaptive}
%==================================================================

\paragraph{The problem.}
Theorem~\ref{thm:conditional} uses $\eta_j^*$ depending on the
unknown per-cell path length $P_T^j$. This section removes that
dependence. We note upfront that the argument below is a \emph{proof
sketch}: the Hedge meta-regret calculation and its propagation through
the main analysis are outlined but not fully carried through. We include
it to indicate the direction of the argument; a complete proof is left
for future work.

\paragraph{Approach.}
For each cell $j$, maintain a Hedge (multiplicative weights) algorithm
over a grid of candidate step sizes $\mathcal{H}=\{2^{-i}:i=0,1,
\dots,\lceil\log_2 T\rceil\}$. At each visit to cell $j$, the active
step size is drawn from the Hedge distribution and the observed coverage
loss $(1-z_k)-\alpha$ is used to update the weights.

\paragraph{Informal rate.}
Standard Hedge analysis over $|\mathcal{H}|=O(\log T)$ experts gives
meta-regret $O(\sqrt{m_j\log\log T})$ per cell relative to the best
fixed step size. Since $m_j^{5/6}\gg\sqrt{m_j}$ for large $m_j$, this
meta-regret is lower order and the main rate is unchanged. Summing over
cells, the additional cost is $O(h^{-d}\sqrt{p_{\min}h^dT\log\log T})
=O(T^{1/2+d/(2(6\beta+d))}(\log T)^{1/2})$, which is lower order than
$T^{(5\beta+d)/(6\beta+d)}$ for all $\beta>0$ (since
$1/2+d/(2(6\beta+d))<(5\beta+d)/(6\beta+d)$ iff $3\beta<5\beta$,
always true for $\beta>0$). Making this fully rigorous would require
verifying the Hedge loss boundedness assumptions and tracing the
propagation of meta-regret through the cell-aggregation argument
in Step 5 above.

%==================================================================
\section{Comparison and Hierarchy}
\label{sec:comparison}
%==================================================================

\begin{center}
\small
\begin{tabular}{lllll}
\hline
Model & Feedback & Target & Coverage metric & $R(T)$\\
\hline
I: Adversarial (Sec.~\ref{sec:adversarial})
  & Full score & Marginal & $Q(T)=O(\sqrt{T(1+P_T)})$ & $O(L\sqrt{T(1+P_T)})$\\
II: Scalar stochastic (Sec.~\ref{sec:scalar})
  & Full score & Marginal & $Q(T)=O(T^{2/3}V_T^{1/3})$ & $O(T^{2/3}V_T^{1/3}/f_{\min})$\\
III: Conditional (Sec.~\ref{sec:conditional})
  & Single bit & Conditional & $V_c(T)=O(T^{(5\beta+d)/(6\beta+d)}P_T^{2\beta/(6\beta+d)})$ &
    $O(L_\mu T^{(5\beta+d)/(6\beta+d)}P_T^{2\beta/(6\beta+d)}/p_{\min}^s)$\\
ACI \cite{gibbs2021}
  & Single bit & Marginal & $O(1/T)$ (signed avg) & ---\\
\hline
\end{tabular}
\end{center}

\paragraph{A note on the coverage-metric column.}
The symbol used for the coverage metric changes with the feedback model,
following the general problem formulation above: $Q(T)$ denotes the
cumulative feasibility violation (Models~I--II, pathwise in Model~I and
its distributional analogue in Model~II), while $V_c(T)$ denotes its
covariate-conditional counterpart in Model~III, where the target itself
is function-valued.

\paragraph{Key observations.}
The three models form a strict difficulty hierarchy.
Model I has no statistical structure; Model II adds stochasticity
and achieves a much better rate but requires full score feedback;
Model III adds conditional coverage and restricts to a single bit.

The gap $T^{2/3}\to T^{5/6}$ (from II to III for $d=0$, $\beta=1$)
is the simultaneous cost of (a) single-bit feedback and (b) conditional
coverage. The $1/f_{\min}$ (or $1/p_{\min}^s$) factor in $R(T)$ across
all settings is information-theoretically necessary: it is the inverse
of the score density at the oracle threshold, measuring how sensitively
coverage responds to threshold changes; if the density is near zero,
even a large threshold error barely affects coverage probability, making
the problem intrinsically harder to notice.

ACI's signed average guarantee is incomparable to our absolute bounds:
it allows cancellation across rounds, which ours do not.

%==================================================================
\section{Discussion}
\label{sec:discussion}
%==================================================================

\paragraph{Lower bound for conditional setting.}
No matching lower bound for the conditional bandit setting ($d>0$,
Model III) is established. For $d=0$, $T^{5/6}$ matches known
rates for one-bit stochastic root-finding under drift (Robbins-Monro
with a drifting root), suggesting the bound may be tight, but this
requires a separate proof.

\paragraph{Fixed score function.}
All settings assume the score function $s$ is fixed. In practice it is
often updated online, creating feedback between score quality and
threshold calibration. Extending to joint score-and-threshold adaptation
is an important open problem.

\paragraph{Exact conditional coverage.}
Barber et al.~\cite{barber2021} showed that exact pointwise conditional
coverage is impossible without strong distributional assumptions.
Our Model III provides marginal bounds on a function-valued target
that approximate conditional coverage, but the gap between marginal and
exact conditional coverage remains.

\paragraph{Finite-time constants.}
All bounds are stated with $O(\cdot)$; tracking explicit constants
(particularly in $p_{\min}^s$, $p_{\max}^s$, and $L_\mu$) is relevant
for practical step-size selection and is left for future work.

